Sparse Plus Low Rank Matrix Decomposition: A Discrete Optimization Approach

We study the Sparse Plus Low-Rank decomposition problem (SLR), which is the problem of decomposing a corrupted data matrix into a sparse matrix of perturbations plus a low-rank matrix containing the ground truth. SLR is a fundamental problem in Operations Research and Machine Learning which arises in various applications, including data compression, latent semantic indexing, collaborative filtering, and medical imaging. We introduce a novel formulation for SLR that directly models its underlying discreteness. For this formulation, we develop an alternating minimization heuristic that computes high-quality solutions and a novel semidefinite relaxation that provides meaningful bounds for the solutions returned by our heuristic. We also develop a custom branch-and-bound algorithm that leverages our heuristic and convex relaxations to solve small instances of SLR to certifiable (near) optimality. Given an input $n$-by-$n$ matrix, our heuristic scales to solve instances where $n=10000$ in minutes, our relaxation scales to instances where $n=200$ in hours, and our branch-and-bound algorithm scales to instances where $n=25$ in minutes. Our numerical results demonstrate that our approach outperforms existing state-of-the-art approaches in terms of rank, sparsity, and mean-square error while maintaining a comparable runtime.

==> Table1_first_old.tex <==
\begin{tabular}{ccc || cc || ccccc}
\toprule
    \multicolumn{3}{c}{} & \multicolumn{2}{c}{} & \multicolumn{5}{c}{L Error} \\
    \cmidrule(l){1-3} \cmidrule(l){4-5} \cmidrule(l){6-10}
    N & $k_0$ & $k_1$ & S-PCP Rank & S-PCP Sparsity &  S-PCP &  GoDec & ScaledGD &  fRPCA &     Alg 1 Exact \\
\midrule
 20 &     1 &    20 &        5.7 &           95.6 & 0.0176 & 0.0101 &   0.0082 & 0.0088 & \textbf{0.0072} \\
 20 &     2 &    40 &       12.0 &          197.4 & 0.0178 & 0.0430 &   0.0062 & 0.0068 & \textbf{0.0057} \\
 20 &     3 &    60 &       15.3 &          275.3 & 0.1123 & 0.1136 &   0.0084 & 0.0077 & \textbf{0.0075} \\
 20 &     4 &    80 &       17.5 &          341.1 & 0.1510 & 0.3247 &   0.0087 & 0.0088 & \textbf{0.0079} \\
 40 &     2 &    80 &        5.4 &          286.6 & 0.0233 & 0.0121 &   0.0147 & 0.0174 & \textbf{0.0110} \\
 40 &     4 &   160 &       16.4 &          417.2 & 0.0272 & 0.0189 &   0.0122 & 0.0136 & \textbf{0.0113} \\
 40 &     6 &   240 &       27.3 &          731.3 & 0.0334 & 0.0996 &   0.0159 & 0.0165 & \textbf{0.0145} \\
 40 &     8 &   320 &       36.7 &         1365.1 & 0.0453 & 0.3225 &   0.0170 & 0.0157 & \textbf{0.0149} \\
 60 &     3 &   180 &        7.8 &          631.6 & 0.0311 & 0.0158 &   0.0182 & 0.0197 & \textbf{0.0149} \\
 60 &     6 &   360 &       13.0 &          777.6 & 0.0328 & 0.0247 &   0.0171 & 0.0177 & \textbf{0.0150} \\
 60 &     9 &   540 &       36.3 &         1181.1 & 0.0439 & 0.0520 &   0.0236 & 0.0226 & \textbf{0.0202} \\
 60 &    12 &   720 &       55.9 &         2930.5 & 0.0577 & 0.2696 &   0.0236 & 0.0242 & \textbf{0.0209} \\
 80 &     4 &   320 &       10.9 &         1128.5 & 0.0345 & 0.0176 &   0.0230 & 0.0238 & \textbf{0.0166} \\
 80 &     8 &   640 &       15.4 &         1380.1 & 0.0448 & 0.0293 &   0.0240 & 0.0248 & \textbf{0.0223} \\
 80 &    12 &   960 &       34.0 &         1634.6 & 0.0569 & 0.0537 &   0.0271 & 0.0269 & \textbf{0.0246} \\
 80 &    16 &  1280 &       62.7 &         3316.8 & 0.0737 & 0.2989 &   0.0339 & 0.0339 & \textbf{0.0300} \\
100 &     5 &   500 &       13.8 &         1771.6 & 0.0443 & 0.0255 &   0.0288 & 0.0267 & \textbf{0.0239} \\
100 &    10 &  1000 &       19.2 &         2139.9 & 0.0531 & 0.0357 &   0.0318 & 0.0345 & \textbf{0.0271} \\
100 &    15 &  1500 &       36.4 &         2525.9 & 0.0640 & 0.0679 &   0.0356 & 0.0330 & \textbf{0.0304} \\
100 &    20 &  2000 &       63.4 &         3145.1 & 0.0840 & 0.3675 &   0.0399 & 0.0395 & \textbf{0.0381} \\
120 &    12 &  1440 &       21.3 &         3067.7 & 0.0644 & 0.0423 &   0.0368 & 0.0400 & \textbf{0.0333} \\
120 &    18 &  2160 &       38.8 &         3628.4 & 0.0789 & 0.0858 &   0.0440 & 0.0424 & \textbf{0.0388} \\
120 &    24 &  2880 &       72.0 &         4288.3 & 0.0968 & 0.3838 &   0.0512 & 0.0498 & \textbf{0.0464} \\
140 &     7 &   980 &       19.3 &         3436.0 & 0.0613 & 0.0365 &   0.0386 & 0.0375 & \textbf{0.0331} \\
140 &    21 &  2940 &       37.9 &         4911.8 & 0.0868 & 0.0910 &   0.0506 & 0.0479 & \textbf{0.0442} \\
140 &    28 &  3920 &       76.7 &         5790.9 & 0.1085 & 0.4156 &   0.0607 & 0.0598 & \textbf{0.0566} \\
\bottomrule
\end{tabular}


==> Table1_second_old.tex <==
\begin{tabular}{ccc || cc || cc ||c}
\toprule
    \multicolumn{3}{c}{} & \multicolumn{2}{c}{L Error} & \multicolumn{2}{c}{Time (s)} & \multicolumn{1}{c}{}\\
    \cmidrule(l){1-3} \cmidrule(l){4-5} \cmidrule(l){6-7} \cmidrule(l){8-8}
    N &  $k_0$ &  $k_1$ & Alg 1 Exact & Alg 1 Acc & Alg 1 Exact & Alg 1 Acc &  Time Decrease (\%) \\
\midrule
 20 &      1 &     20 & \textbf{0.0072} &              0.0245 &         0.2044 &      \textbf{0.0834} \\
 20 &      2 &     40 & \textbf{0.0059} &              0.0165 &         0.2746 &      \textbf{0.0858} \\
 20 &      3 &     60 & \textbf{0.0064} &              0.0169 &         0.2926 &      \textbf{0.1189} \\
 20 &      4 &     80 & \textbf{0.0080} &              0.0175 &         0.3353 &      \textbf{0.1358} \\
 40 &      2 &     80 & \textbf{0.0108} &              0.0471 &         0.5863 &      \textbf{0.2226} \\
 40 &      4 &    160 & \textbf{0.0116} &              0.0537 &         0.9146 &      \textbf{0.2320} \\
 40 &      6 &    240 & \textbf{0.0151} &              0.0554 &         1.1864 &      \textbf{0.2720} \\
 40 &      8 &    320 & \textbf{0.0171} &              0.0521 &         1.5017 &      \textbf{0.3037} \\
 60 &      3 &    180 & \textbf{0.0145} &              0.0717 &         0.6818 &      \textbf{0.3693} \\
 60 &      6 &    360 & \textbf{0.0163} &              0.0716 &         1.8328 &      \textbf{0.3813} \\
 60 &      9 &    540 & \textbf{0.0199} &              0.0810 &         0.8734 &      \textbf{0.3869} \\
 60 &     12 &    720 & \textbf{0.0208} &              0.0771 &         0.9200 &      \textbf{0.4264} \\
 80 &      4 &    320 & \textbf{0.0159} &              0.1028 &         1.0392 &      \textbf{0.4843} \\
 80 &      8 &    640 & \textbf{0.0220} &              0.1230 &         1.1944 &      \textbf{0.5212} \\
 80 &     12 &    960 & \textbf{0.0248} &              0.1277 &         1.4087 &      \textbf{0.5486} \\
 80 &     16 &   1280 & \textbf{0.0292} &              0.1342 &         1.6078 &      \textbf{0.5671} \\
100 &      5 &    500 & \textbf{0.0227} &              0.1483 &         1.7150 &      \textbf{0.8052} \\
100 &     10 &   1000 & \textbf{0.0268} &              0.1655 &         1.9810 &      \textbf{0.8014} \\
100 &     15 &   1500 & \textbf{0.0300} &              0.1825 &         2.3986 &      \textbf{0.9207} \\
100 &     20 &   2000 & \textbf{0.0348} &              0.1837 &         3.1043 &      \textbf{1.0324} \\
120 &      6 &    720 & \textbf{0.0279} &              0.2151 &         2.2287 &      \textbf{0.9986} \\
120 &     12 &   1440 & \textbf{0.0332} &              0.2375 &         2.6314 &      \textbf{1.1321} \\
120 &     18 &   2160 & \textbf{0.0384} &              0.2581 &         3.0367 &      \textbf{1.2760} \\
120 &     24 &   2880 & \textbf{0.0434} &              0.2767 &         4.1622 &      \textbf{1.2622} \\
140 &      7 &    980 & \textbf{0.0326} &              0.2688 &         3.4058 &      \textbf{2.4650} \\
140 &     14 &   1960 & \textbf{0.0370} &              0.3030 &         3.7347 &      \textbf{1.5876} \\
140 &     21 &   2940 & \textbf{0.0438} &              0.3275 &         4.4423 &      \textbf{1.6191} \\
140 &     28 &   3920 & \textbf{0.0530} &              0.3833 &         6.4438 &      \textbf{1.5769} \\
\bottomrule
\end{tabular}


==> Table1_third_old.tex <==
\begin{tabular}{ccc || ccccc || cc}
\toprule
    \multicolumn{3}{c}{} & \multicolumn{5}{c}{L Error} & \multicolumn{2}{c}{} \\
    \cmidrule(l){1-3} \cmidrule(l){4-8} \cmidrule(l){9-10}
    N & $k_0$ & $k_1$ & S-PCP & GoDec & ScaledGD & fRPCA & Alg 1 Exact & Alg 1 Bound Gap & Bound Time (s) \\
\midrule
 20 &     1 &    20 & 0.0176 & 0.0101 &   0.0082 & 0.0088 & \textbf{0.0072} &          0.7052 &         3.7200 \\
 60 &     6 &   360 & 0.0328 & 0.0247 &   0.0171 & 0.0177 & \textbf{0.0150} &          0.8543 &       189.1900 \\
 60 &     9 &   540 & 0.0439 &  0.052 &   0.0236 & 0.0226 & \textbf{0.0202} &          0.8601 &       184.9500 \\
 60 &    12 &   720 & 0.0577 & 0.2696 &   0.0236 & 0.0242 & \textbf{0.0209} &          0.7709 &       155.2800 \\
 80 &     4 &   320 & 0.0345 & 0.0176 &   0.0230 & 0.0238 & \textbf{0.0166} &          0.9180 &       577.8400 \\
 80 &     8 &   640 & 0.0448 & 0.0293 &   0.0240 & 0.0248 & \textbf{0.0223} &          0.9267 &       765.9100 \\
 80 &    12 &   960 & 0.0569 & 0.0537 &   0.0271 & 0.0269 & \textbf{0.0246} &          0.7944 &       691.5500 \\
 80 &    16 &  1280 & 0.0737 & 0.2989 &   0.0339 & 0.0339 & \textbf{0.0300} &          0.7803 &       611.4700 \\
100 &     5 &   500 & 0.0443 & 0.0255 &   0.0288 & 0.0267 & \textbf{0.0239} &          0.9592 &      1936.2600 \\
100 &    10 &  1000 & 0.0531 & 0.0357 &   0.0318 & 0.0345 & \textbf{0.0271} &          0.9382 &      2987.0800 \\
100 &    15 &  1500 &  0.064 & 0.0679 &   0.0356 & 0.0330 & \textbf{0.0304} &          0.9062 &      2224.6100 \\
 20 &     2 &    40 & 0.0178 &  0.043 &   0.0062 & 0.0068 & \textbf{0.0057} &          0.5935 &         3.8200 \\
100 &    20 &  2000 &  0.084 & 0.3675 &   0.0399 & 0.0395 & \textbf{0.0381} &          0.8145 &      2188.6600 \\
120 &    12 &  1440 & 0.0644 & 0.0423 &   0.0368 & 0.0400 & \textbf{0.0333} &          0.8951 &      6759.9200 \\
120 &    18 &  2160 & 0.0789 & 0.0858 &   0.0440 & 0.0424 & \textbf{0.0388} &          0.8968 &      6878.3600 \\
120 &    24 &  2880 & 0.0968 & 0.3838 &   0.0512 & 0.0498 & \textbf{0.0464} &          0.7877 &      5310.5800 \\
140 &     7 &   980 & 0.0613 & 0.0365 &   0.0386 & 0.0375 & \textbf{0.0331} &          0.9014 &     14731.2500 \\
140 &    21 &  2940 & 0.0868 &  0.091 &   0.0506 & 0.0479 & \textbf{0.0442} &          0.8854 &     11260.5200 \\
140 &    28 &  3920 & 0.1085 & 0.4156 &   0.0607 & 0.0598 & \textbf{0.0566} &          0.8116 &     11840.3000 \\
 20 &     3 &    60 & 0.1123 & 0.1136 &   0.0084 & 0.0077 & \textbf{0.0075} &          0.5443 &         3.9600 \\
 20 &     4 &    80 &  0.151 & 0.3247 &   0.0087 & 0.0088 & \textbf{0.0079} &          0.7146 &         4.0500 \\
 40 &     2 &    80 & 0.0233 & 0.0121 &   0.0147 & 0.0174 & \textbf{0.0110} &          0.8214 &        30.6200 \\
 40 &     4 &   160 & 0.0272 & 0.0189 &   0.0122 & 0.0136 & \textbf{0.0113} &          0.8804 &        27.9200 \\
 40 &     6 &   240 & 0.0334 & 0.0996 &   0.0159 & 0.0165 & \textbf{0.0145} &          0.7937 &        28.4700 \\
 40 &     8 &   320 & 0.0453 & 0.3225 &   0.0170 & 0.0157 & \textbf{0.0149} &          0.7051 &        23.8700 \\
 60 &     3 &   180 & 0.0311 & 0.0158 &   0.0182 & 0.0197 & \textbf{0.0149} &          0.8075 &       154.9000 \\
\bottomrule
\end{tabular}


==> Table9_old.tex <==
\begin{tabular}{c c c || ccc || ccc || ccc}
\toprule
    \multicolumn{3}{c}{} & \multicolumn{3}{c}{L Error} & \multicolumn{3}{c}{S Error} & \multicolumn{3}{c}{Time (s)}\\
    \cmidrule(l){1-3} \cmidrule(l){4-6} \cmidrule(l){7-9} \cmidrule(l){10-12}
    N & $k_0$ & $k_1$ & Alg 1 Exact & GoDec & ScaledGD & Alg 1 Exact & GoDec & ScaledGD & Alg 1 Exact & GoDec & ScaledGD \\
  200 &     \textbf{0.0442} &        0.0458 &           0.0450 &     \textbf{0.5677} &        0.9246 &           0.7432 &      \textbf{0.0185} &          0.0187 &            4.4279 \\
  250 &     \textbf{0.0538} &        0.0553 &           0.0545 &     \textbf{0.6176} &        1.0208 &           0.7476 &      \textbf{0.0191} &          0.0250 &            6.7974 \\
  300 &     \textbf{0.0641} &        0.0654 &           0.0646 &     \textbf{0.6725} &        1.1036 &           0.7812 &               0.0314 & \textbf{0.0290} &           10.1082 \\
  350 &     \textbf{0.0755} &        0.0766 &           0.0759 &     \textbf{0.7307} &        1.1955 &           0.8337 &               0.0436 & \textbf{0.0411} &           13.5718 \\
  400 &     \textbf{0.0852} &        0.0863 &           0.0855 &     \textbf{0.7716} &        1.2483 &           0.8664 &               0.0574 & \textbf{0.0517} &           18.4740 \\
  450 &     \textbf{0.0970} &        0.0980 &           0.0974 &     \textbf{0.8038} &        1.2918 &           0.9228 &               0.0792 & \textbf{0.0712} &           24.4337 \\
  500 &     \textbf{0.1083} &        0.1093 &           0.1088 &     \textbf{0.8530} &        1.3585 &           0.9846 &      \textbf{0.0906} &          0.0918 &           29.5441 \\
  550 &     \textbf{0.1213} &        0.1222 &           0.1218 &     \textbf{0.8918} &        1.4021 &           1.0625 &               0.1138 & \textbf{0.1049} &           33.7424 \\
  600 &     \textbf{0.1322} &        0.1331 &           0.1327 &     \textbf{0.9377} &        1.4593 &           1.1322 &      \textbf{0.1357} &          0.1384 &           37.1889 \\
  650 &     \textbf{0.1430} &        0.1438 &           0.1437 &     \textbf{0.9624} &        1.4842 &           1.2020 &      \textbf{0.1538} &          0.1693 &           45.6313 \\
  700 &     \textbf{0.1554} &        0.1562 &           0.1560 &     \textbf{1.0126} &        1.5524 &           1.2872 &      \textbf{0.1810} &          0.2022 &           54.8570 \\
  750 &     \textbf{0.1681} &        0.1689 &           0.1687 &     \textbf{1.0244} &        1.5587 &           1.3556 &      \textbf{0.3668} &          0.5669 &           67.4488 \\
  800 &     \textbf{0.1812} &        0.1820 &           0.1820 &     \textbf{1.0676} &        1.6062 &           1.4383 &      \textbf{0.3395} &          0.5000 &           90.5553 \\
  850 &     \textbf{0.1918} &        0.1925 &           0.1925 &     \textbf{1.0967} &        1.6372 &           1.5294 &      \textbf{0.9337} &          1.0395 &          346.6197 \\
  900 &     \textbf{0.2057} &        0.2064 &           0.2065 &     \textbf{1.1348} &        1.6852 &           1.6192 &               1.7587 & \textbf{1.5853} &          521.5712 \\
  950 &     \textbf{0.2174} &        0.2181 &           0.2184 &     \textbf{1.1543} &        1.6942 &           1.6956 &               0.7749 & \textbf{0.7494} &          779.0286 \\
 1000 &     \textbf{0.2306} &        0.2313 &           0.2314 &     \textbf{1.1783} &        1.7207 &           1.7794 &               3.2104 & \textbf{3.1600} &         1095.0363 \\
 2000 &     \textbf{0.5171} &        0.5177 &           0.5189 &     \textbf{1.5707} &        2.1098 &           3.6432 &               1.3195 & \textbf{1.3155} &          565.8465 \\
 4000 &     \textbf{1.3013} &        1.3019 &           1.3050 &     \textbf{2.1207} &        2.6438 &           8.0121 &     \textbf{35.1148} &         36.9398 &        11777.4625 \\
 6000 &     \textbf{2.3694} &        2.3700 &           2.3752 &     \textbf{2.3058} &        2.7742 &          11.9628 &     \textbf{84.7058} &         87.7330 &        36950.0315 \\
 8000 &     \textbf{3.5365} &        3.5373 &           3.5400 &     \textbf{2.5880} &        3.0463 &          16.9418 &    \textbf{158.5785} &        160.0202 &        68606.5505 \\
10000 &     \textbf{4.8465} &        4.8472 &           4.8547 &     \textbf{2.7586} &        3.1967 &          21.6143 &    \textbf{133.3238} &        145.8102 &       110806.3610 \\
\bottomrule
\end{tabular}

